GNUMAP: A Parameter-Free Approach to Unsupervised Dimensionality Reduction via Graph Neural Networks

With the proliferation of Graph Neural Network (GNN) methods stemming from contrastive learning, unsupervised node representation learning for graph data is rapidly gaining traction across various fields, from biology to molecular dynamics, where it is often used as a dimensionality reduction tool. However, there remains a significant gap in understanding the quality of the low-dimensional node representations these methods produce, particularly beyond well-curated academic datasets. To address this gap, we propose here the first comprehensive benchmarking of various unsupervised node embedding techniques tailored for dimensionality reduction, encompassing a range of manifold learning tasks, along with various performance metrics. We emphasize the sensitivity of current methods to hyperparameter choices -- highlighting a fundamental issue as to their applicability in real-world settings where there is no established methodology for rigorous hyperparameter selection. Addressing this issue, we introduce GNUMAP, a robust and parameter-free method for unsupervised node representation learning that merges the traditional UMAP approach with the expressivity of the GNN framework. We show that GNUMAP consistently outperforms existing state-of-the-art GNN embedding methods in a variety of contexts, including synthetic geometric datasets, citation networks, and real-world biomedical data -- making it a simple but reliable dimensionality reduction tool.

==> benchmark-gnn-methods.tex <==
Representation learning on graphs is an area of active research nowadays. %There are also rather traditional approaches based on graph theory, but this paper focuses on GNN as a graph representation learning tool. 
Deep graph embedding can not only use the topological features over the graph but also incorporate the feature information by the message-passing scheme. In this section, we will review the existing GNN models which can be used for dimensionality reduction. The methods should be unsupervised in its nature, as we want to use the resulting embedded vectors for visualization to detect the cluster, interpret the structure, and so on. Then, we propose a novel GNN architecture: \textit{gnumap}. \textit{gnumap} is also a self-supervised contrastive learning model, with cross-entropy loss. Unlike existing GNN architectures, this model is designed toward dimensionality reduction and visualization.  



\subsection{Related Works}
% https://github.com/cxtmavro/awesome-unsupervised-gnns
\subsubsection{Graph Autoencoder(GAE)}
Variational Graph Autoencoder\cite{vgae2016kipf} is an extension of Variational Autoencoder\cite{Kingma2013VAE}. Graph Autoencoder(GAE) is non-probabilistic version of VGAE. Let us denote the reconstructed adjacency matrix as $\hat{\matbf{A}}$.
\begin{enumerate}
    \item Encoder: $\mathbf{Y}  = \text{GCN}(\mathbf{X}, \mathbf{A})$, where $\text{GCN}(\mathbf{X}, \mathbf{A}) = \tilde{\mathbf{A}}\text{ReLU}(\tilde{\mathbf{A}}\mathbf{X}W_0)W_1$ is defined as two-layer GCN, and $\tilde{\mathbf{A}} = D^{-1/2}\mathbf{A} D^{-1/2}$, a normalized adjacency matrix.
    \item Decoder: $\hat{\mathbf{A}} = \sigma(\mathbf{Y},\mathbf{Y}^\top)$, $\sigma(\cdot)$ is a sigmoid function.
    \item Loss for positive edges(loss\_pos): $-\frac{1}{|\mathcal{E}|}\sum_{e_{ij} \in \mathcal{E}}\big[ \log(\sigma(\mathbf{y_i}^\top\mathbf{y_j})+\epsilon \big]$
    \item Loss for negative edges(loss\_neg): $-\frac{1}{N}\sum_{e_{ij} \notin \mathcal{E}}\big[ \log(1 - \sigma(\mathbf{y_i}^\top\mathbf{y_j})+\epsilon \big]$, where N is the number of negative edges used for the training.
    \item loss = loss\_pos + loss\_neg; the binary cross entropy loss.
    \item Optimization: apply Adam\cite{Kingma2014Adam} optimizer, with a learning rate 0.01.
\end{enumerate}

\subsubsection{Deep Graph Contrastive Representation Learning(GRACE)}
Contrastive learning or self-supervised method has gotten increasing attention as they do not require label availability as supervised GNN does. Deep Graph Contrastive Representation Learning(GRACE)\cite{grace} is one of the popular graph constrastive learning methods.
\begin{enumerate}
    \item For each iteration, GRACE generates two graph views, $\tilde{G_1}, \tilde{G_2}$, by either randomly removing edges or randomly masking node features. 
    \item Let $U = f(\tilde{X_1}, \tilde{A_1}), V = f(\tilde{X_2}, \tilde{A_2})$ be the embedded representation of two graph views, and their corresponding node features and adjacency matrices. 
    \item Positive samples: For any node $v_i$, its corresponding representation in another view $u_i$ is treated as natural positive pair. 
    \item Negative samples: For given node $v_i$, any nodes in another view $u_{k \neq i}$ are treated as negative pair. 
    \item Node-wise objective: $$ \ell(u_i, v_i) = \text{log} \frac{ e^{\theta(u_i,v_i)/ \tau}} { \underbrace{e^{\theta(u_i,v_i)/\tau}}_\text{the positive pair} + \underbrace{\sum_{k=1}^N \mathbbm{1}_{k \neq i} e^{\theta (u_i,v_k)/\tau}}_\text{inter-view negative pairs} + \underbrace{\sum_{k=1}^N\mathbbm{1}_{k \neq i} e^{\theta(u_i,u_k)/\tau}}_\text{intra-view negative pairs} } $$
    \item Overall loss function: $\ell = \frac{1}{2N}\sum_{i=1}^N \big[\ell(u_i, v_i) + \ell(v_i, u_i) \big]$
    \item Optimization: apply stochastic gradient descent.
\end{enumerate}

%\subsubsection{Contrastive Multi-View Representation Learning on Graphs(MVGRL)}

\subsubsection{Deep Graph Infomax(DGI)}
\cite{stokes2020deep}

\subsubsection{Large-Scale Representation Learning on Graphs via Bootstrapping(BGRL)}
\cite{thakoor2023largescale}

\subsubsection{From Canonical Correlation Analysis to
Self-supervised Graph Neural Networks(CCA-SSG)}
\cite{zhang2021canonical}




==> metrics.tex <==
\subsection{Evaluation Metrics}
Our primary purpose is to show the advantages and disadvantages of GNN compared to other dimension reduction methods. We want the embeddings in a lower dimensional space to preserve the global, local geometry of the original data, as well as the density information. Also, we hope the method is robust to the noise and initialization of embeddings. Lastly, the method is better if its algorithm is efficient in incorporating an increasing number of features(p) and samples(n).


\subsubsection{Global Geometry}
We hope the dimension reduction method preserves the global geometry of the original data. Good representation would retain the global structure of the original data so that their pairwise distance is somewhat preserved, which will be evaluated by the Spearman correlation coefficient in our setting. When it comes to a supervised setting, the desirable properties would be well separate the distinctive cluster by a linear classifier such as Support Vector Machine(SVM) or linear regression.

\xhdr{Supervised Learning}\label{global-supervised}
We hope our low-dimensional space can form well-separated clusters for the supervised setting. To evaluate the performance, we either use classification accuracy or adjust $R^2$ depending on the data. 
\begin{enumerate}
    \item We use k-fold cross-validation to fit the model and evaluation metric. For the experiment, $k = 10$ was used. 
    \item Fit the model; label or the independent variable is given with true value, and dependent variables are given as our low-dimensional embedding.
    \item For the classification setting, we use Support Vector Machine(SVM) with default rbf kernel. For the regression setting, we use adjusted $R^2$ for the linear regression model. 
    \item The evaluated classification accuracy or $R^2$ will be averaged over the folds. 
\end{enumerate}
%Silhouette coefficient

\xhdr{Unsupervised Learning}
We measure the amount of preservation in global structure by using a Spearman correlation between the pairwise distance in high-dimensional embedding space and embedding space from the model. If the value of correlation is closer to 1, we could say that our embedding spaces resemble the perfect embedding space, which is known to preserve the geometry of the graphs in a lower dimension. Inspired by Isomap\cite{isomap}, the pairwise distance in the original space is evaluated by the shortest-path distance over the (given/reconstructed) graph, assuming that the geodesic distance on the manifold can be reasonably approximated by the shortest-path distance. The pairwise distance in the projected space is evaluated by standard euclidean distance.

% Wasserstein loss can be an alternative metric to evaluate the global structure.


\subsubsection{Local Geometry}
We also want the embedding space that preserves the local structure of the data. We want the points in a cluster neighboring each other in the original data to stay in proximity on the embedding space. 

Inspired by \cite{Huang2022DREval}, we measure it by the percentage of overlap by K-nn graphs on the embedding space. We construct the K-nn graphs on the embedding space and see how many nodes from each node stay connected on the embedding space compared to the original graph or knn-graph from the original data, i.e. $$\frac{1}{n}\sum_{i=1}^{n}\frac{\text{\# of overlapping neighborhood on } x_i}{\text{node degree}(x_i)}$$

\subsubsection{Density Preservation}
We hope to preserve the density from the original space in the embedding space. That is, we want dense clusters from the original space to be projected more concentrated in the embedding space and sparse clusters in a more scattered manner.

\xhdr{Defintion} Motivated by the concept provided in \cite{densmap}, we will evaluate the correlation of \textit{local radius} between the original and embedding spaces.
\begin{enumerate}
    \item Let $P$, $Q$ be the distribution of edge weight or probability of node connection on original and embedding space, respectively. For example, given $x_i$ and $x_j$ are connected, $p_{ij}$ is the probability of node $x_i$ and $x_j$ being connected. 
    \item Let local radius $R_p(x_i) = \frac{p_{ij}}{\sum_j p_{ij}} \sum_j p_{ij} d(x_i, d_j)$. The local radius on the embedding space can also be defined in an analogous way with distribution Q. 
    \item We hope the local radius on original space and embedding space to have \textit{power-law} relationship, i.e. $R_e(y_i) \approx R_o(x_i)$. Let $r_o(x_i): = log(R_o(x_i)$, $r_e(y_i): = log(R_e(y_i)$
    \item Finally, the goodness-of-fit can be measured by $Corr(r_o,r_e)$.
\end{enumerate}
\xhdr{Intuition}
The intuition behind this measure defined on \cite{densmap} is that given a point, if the expected distance to the neighborhood is small then the point should be classified as a "dense" point, and vice versa. In the original paper, they follow the UMAP\cite{umap}, t-SNE\cite{tsne-theory} way of defining the probability density on high-dimensional and low-dimensional space. Here, if we are given edge weight, then high-dimensional probability will be substituted with the edge weight; otherwise, we will follow the UMAP version.

\subsubsection{Scalability with the Sample size(n)} 
We evaluate the scalability of each method with respect to the sample size(n) by computational efficiency. This can be easily measured by the runtime of each algorithm on different sample sizes. For the visual inspection, we will provide the line plot. For the numerical inspection, we will provide the slope between the sample size and the runtime. 

% source: https://umap-learn.readthedocs.io/en/latest/benchmarking.html
%\xhdr{Analysis}
%t-SNE not scalable because of the denominator. UMAP is better than t-SNE. GNN scales well with the size of the graph, as the weight and bias are usually shared in commonly used aggregation scheme(GCN, GAT, Graph SAGE) PCA scale not well, need matrix decomposition \todo[inline]{add citations and formulas}

\subsubsection{Scalability with the Dimension(p)}
We test the performance of the benchmark methods by varying the dimension of the data. We may use PCA(Principal Component Analysis) to adjust the input dimension. By increasing the dimension, we want to see how the performance of each method varies, with particular interests in runtime and global geometry metrics. We will use the data of dimension(p) large enough, so that we can control the dimension size with PCAs, for example, MNIST, Fashion MNIST, and CIFAR10 dataset, all of which are loaded using \verb|sklearn.datasets.fetch_openml|.

From a preliminary analysis of the datasets, we figured the number of PCs needed to explain 50\%, 80\%, 90\% of the entire variance to determine the reasonable number of features for the experiments.

%\xhdr{Analysis} \todo[inline]{add discussions}
\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{figures/mnist_with_diff_p.png}
    \caption{Experiments on MNIST with varying number of PCs as an input.}
    \label{fig:my_label}
\end{figure}

\subsubsection{Robustness to Initialization}
One of the most popular choices for the initialization is (1) log normalization (2) PCA, and (3) both. We prefer the method robust to the initialization.\cite{metrics} We used the performance quality with different initialization methods using the given options available. For t-SNE, we try two options available from \verb|sklearn.manifold.TSNE|: PCA and random initialization. For UMAP, we also tested two out of three available options at \verb|umap.umap_.UMAP|: PCA and random initialization. Note that the default initialization method used for UMAP is spectral embedding. 
For GNN model, we try a number of weight initialization methods as a proxy for the embedding initialization provided by \verb|torch.nn.init|: \verb|torch.nn.init.normal_()|, \verb|torch.nn.init.xavier_uniform_()| and \verb|torch.nn.init.xavier_ones_()|

\xhdr{Analysis}
It is known that UMAP and t-SNE are not robust to the initialization. Especially, as perplexity increases, the gradient of t-SNE becomes closer to 0, which in return provides an embedding not much different from the initialized one. 
% https://towardsdatascience.com/tsne-vs-umap-global-structure-4d8045acba17 
\todo[inline]{add equations on t-SNE and derive the analogous gradient for UMAP}

\subsubsection{Robustness to Noise}
We will use the synthetic dataset where we can control the amount of noise, for example, circles(\verb|sklearn.datasets.make_circles|), or moons(\verb|sklearn.datasets.make_moons|) can be used for the evaluation. With a varying amount of noise added to the core structure, we want to see how well the clusters are separated from each algorithm. The relative performance will be evaluated by the supervised global geometry metrics that we defined in Section-\ref{global-supervised}, where the baseline is set to be the performance of the data without any noise. For visual inspection, we will provide a line plot of the amount of noise against the performance metric. We will also provide the slope between the noise and the performance for numerical evaluation. 

\xhdr{Analysis}
PCA is good at denoising the data(extract the signal from the data), thus, is robust to the noise. t-SNE and UMAP's robustness depends on the perplexity and the number of neighbors, respectively; if we choose to have a large perplexity or number of neighbors, the algorithms focus on the global geometry of the data, rather than its local noise. However, when such parameters are not large enough, the method would be sensitive to noise. 
%gnumap as a dr for grid-type data--same as umap and t-sne.
%gnumap as a visualizer for the given graph: how to add noise on graphs? 

==> trad-dm-methods-review.tex <==
 As dimensionality reduction is a core topic in Statistics, myriad methods have been proposed to solve this problem. In this section, we will review the most widely used dimensionality reduction algorithm for visualization, focusing on their advantages, disadvantages, and learning mechanisms.
 
 The most famous and well-grounded method is Principal Component Analysis(PCA)\cite{PCA1901Pearson}. PCA has a low computational cost and is designed to retain the maximal information from the original data. However, it works poorly on non-linear data. There are multiple approaches\cite{PrincipalCurve}\cite{PrincipalManifold} to overcome this limitation of PCA. Also, some of the works like Isomap\cite{isomap}, Locally Linearly Embedding(LLE)\cite{LLE}, and Laplacian Eigenmap\cite{LaplacianEigenmap} rely on graphs to recover the manifold structure or non-linear structure of the original dataset. As for recent works, t-SNE\cite{tsne} and UMAP\cite{umap} are among the most popular choices, and they are good at preserving the local geometry, or the points clustered with each other. UMAP works better on balancing between the local and global structure in that it is better at preserving the distance between the clusters. On the other hand, t-SNE is good at preserving the distance within the cluster or preserving the cluster itself, but the distance between the clusters on t-SNE embedding is largely unreliable. Even though t-SNE and UMAP improve a lot from PCA in that they can capture the non-linear structure of high-dimensional data, there is still room to improve. dens-MAP\cite{densmap} again adds a density preservation term on the loss function to preserve the different densities among the clusters.

For consistency, we will use the following notation for the rest of our paper. 
\begin{itemize}
    \item $\mathbf{X} \in \mathcal{R}^{n \times p}$: original grid-type dataset with $n$ samples and $p$ features. $x_i$ denotes each data point.
    \item $\mathcal{G} = \{\mathcal{V}, \mathcal{E}, A\}$, $|\mathcal{V}| = n$, $|\mathcal{E}| = m$: original graph dataset, with $n$ vertices, $m$ edges, $p$ node features. Let each vertex as $x_i, i = 1...n$. The node feature matrix will be denoted as $\mathbf{X} \in \mathcal{R}^{n \times p}$.
    \item $\mathbf{Y} \in \mathcal{R}^{n \times q}$: embedding data in a lower dimensional space of dimension $q < p$. $y_i$ denotes each data point.
    \item $\mathbf{P}$ be the distribution of pairwise connection in the original space of dimension $p$. $p_{ij}$ be the probability of points $x_i$ and $x_j$ being connected.
    \item $\mathbf{Q}$ be the distribution of pairwise connection in the original space of dimension $q$. $q_{ij}$ be the probability of points $y_i$ and $y_j$ being connected.
\end{itemize}

\vspace{5mm}
%==============================
\subsection{Principal Component Analysis(PCA)}
%==============================
Principal Component Analysis\cite{PCA1901Pearson} is a traditional statistical method used for various purposes including dimension reduction. Principal Component(PC) is the orthogonal linear transformation from the original data providing the largest variance. PCA is not scale invariant, thus scaling should be performed before calculating PCs.

\begin{enumerate}
    \item Let us assume that our $X$ has column mean 0, and column-wise standard deviation 1. Otherwise, we need to scale the data before moving onto the next step.
    \item Calculate the singular value decomposition(SVD) of $\mathbf{X}$. 
    $\mathbf{X} = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^\top$ where $\mathbf{U} \in \mathcal{R}^{n \times n}$, of which column is left-singular vector, $\matchbf{V} \in \mathcal{R}^{p \times p}$, a right-singular vector, and $\mathcal{\Simga} \in \mathcal{R}^{n \times p}$, whose diagonal elements are singular values.
    \item Eigenvalue decomposition(EVD) of the covariance matrix of $\mathbf{X}$ can be easily calculated as: $$\mathbf{X}^\top\mathbf{X} = \mathbf{V}\mathbf{\Sigma}^2\mathbf{V}^\top \in \mathcal{R}^{p \times p}$$
    \item Then, the first $q < p$ PCs are given by $\mathbf{T}_q = \mathbf{U}_q\mathbf{\Sigma}_q$, where $\mathbf{U}_q \in \mathcal{R}^{n \times q}$, $\mathbf{\Sigma}_q \in \mathcal{R}^{q \times q}$ are truncated matrices. 
    \item The corresponding eigenvalues for these PCs are given by the diagonal elements of $\mathbf{\Sigma}^2$. This can also be interpreted as  the amount of variance explained by this particular PC. 
\end{enumerate}

\vspace{5mm}
%==============================
\subsection{Isometric Feature Mapping(Isomap)}
%==============================
Combining the major algorithms for linear dimensionality reduction, PCA and Multidimensional Scaling(MDS), the complete isometric feature mapping(Isomap)\cite{isomap} preserves the intrinsic geometry of the data by estimating geodesic distances between the faraway points.
\begin{enumerate}
     \item Connect each points either on their distance, if $\|x_i - x_j\|<\epsilon$($\epsilon$-Isomap) where $\epsilon >0$ is predefined value, or based on k-nearest scheme(K-Isomap).
     \item Calculate the shortest distance, $d_G(i,j)$ over constructed graph $\mathcal{G}$ for connected nodes. The geodesic distance can be approximated for faraway points by the shortest path distance over a graph. 
     \item Let $D_G$ be the distance matrix over the constructed graph, and $D_Y$ be the pairwise distance matrix in the embedding space. Apply MDS to find the lower dimensional embedding in the euclidean space by minimizing $$E = \|\mathbf{f}(D_G) - \mathbf{D}_\mathbf{Y}\|_{L_2}$$. If $\mathbf{f}$ is a linear map, then the minimizer is known to be top q eigenvectors of the matrix $\mathbf{f}(D_G)$.
\end{enumerate}

\vspace{5mm}
%==============================
\subsection{Locally Linearly Embedding(LLE)}
%==============================
Unlike MDS or Isomap, which require calculating the pairwise distance of data points, locally linearly embedding\cite{LLE} reveals nonlinear global structure from locally linear fits. The assumption is that in the reconstructed graph, the data point and its neighbors would lie on or close to a locally linear patch of the manifold. 

\begin{enumerate}
    \item Construct the graph from the given dataset $\mathbf{X}$, simply by applying K nearest neighbors. 
    \item Compute the edge weight by solving the least-squares problem in $\epsilon(W) \sum_i |\mathbf{X}_i - \sum_j \mathbf{W}_{ij}\mathbf{X}_j|^2$.
    \item Given $\hat{\mathbf{W}}$, calculate the low-dimensional embedding $\mathbf{Y}$ by minimizing $\Phi(\mathbf{Y}) = \sum_i|\mathbf{Y_i}-\sum_j \hat{\mathbf{W}}_{ij}\mathbf{Y}_j|^2$. 
\end{enumerate}


\vspace{5mm}
%==============================
\subsection{Laplacian Eigenmaps}
%==============================
Laplacian Eigenmaps\cite{LaplacianEigenmap} tries to preserve the local information by constructing graphs from original data, which assumes to be sampled from the smooth manifold. 
\begin{enumerate}
    \item Connect each points either on their distance, if $\|x_i - x_j\|<\epsilon$ where $\epsilon >0$ is predefined value, or based on k-nearest scheme.
    \item The graph can either be weighted or unweighted. If weighted, the weight is defined by heat kernel, $w_ij = e^{-\frac{\|x_i-x_j\|^2}{t}}$.
    \item Let our reconstructed graph be $\mathcal{G}$, and $L = D - A$ be the corresponding Laplacian matrix. Compute eigenvalues and eigenvectors for the generalized eigenvector problem, $$L\mathbf{f} = \lambda D \mathbf{f}$$
    \item Let $\mathbf{f}_0,\dots, \mathbf{f}_{p-1}$ be the solutions for the eigenvector problems with corresponding eigenvalues $0 = \lambda_0 = \dots = \lambda_{p-1}$. Then $\big(\mathbf{f}_1(i), \dots, \mathbf{f}_q(i)\big)$ becomes q-dimensional embeddings of $x_i$.
\end{enumerate}


\vspace{5mm}
%==============================
\subsection{t-distributed Stochastic Neighbor Embedding(t-SNE)}
%==============================

\vspace{4mm} 
t-SNE\cite{tsne} follows similar logic as UMAP, but the way they define the probability on high and lower dimensional space, and loss function are different than UMAP. Two practical tricks have been used: (1) Early exaggeration (2) embedding stage.
%\todo[inline]{add explanation on tricks for training \cite{tsne-theory}}
\begin{enumerate}
    \item Consider two points i and j. Define the conditional probability $p_{j|i} = \frac{e^{-\|x_i-x_j\|^2/2\sigma_i^2}}{\sum_{k \neq i}e^{-\|x_i-x_k\|^2/2\sigma_i^2}}$ where $\sigma_i$ is computed by applying a binary search to solve the equation: $$\text{Perplexity} = 2− \sum_j p_{j|i} log_2 p_{j|i}$$. The user-defined parameter Perplexity is monotonically increasing in $\sigma_i$. Intuitively, as Perplexity becomes larger, the probabilities become uniform. When Perplexity becomes smaller, the probabilities concentrate heavily on the nearest points.
    \item Define the symmetric probability $p_{ij} = \frac{p_{i|j} +p_{j|i}}{2n}$ . Observe that this probability does not depend on the decision variables $\mathbf{Y}$ and is derived from $\mathbf{X}$
    \item Define the probability $q_{ij} = \frac{(1+\|y_i-y_j\|^2)^{-1}}{\sum_{k \neq l}(1+\|y_k-y_l\|^2)^{-1}} $. Observe that this probability is a function of the decision variables $\mathbf{Y}$.
    \item Define the loss function as $\sum_i \sum_j p_{ij} log \frac{p_{ij}}{q_{ij}}$
    \item Initialization: initialize $\mathbf{Y}$ using the multivariate Normal distribution $\mathcal{N}(0,10^{−4}I)$, with I denoting the q-dimensional identity matrix.
    % \item Optimization: apply gradient descent with momentum. The momentum term is set to 0.5 for the first 250 iterations, and to 0.8 for the following 750 iterations. The learning rate is initially set to 100 and updated adaptively.
\end{enumerate}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline  & \textbf{t-SNE}                                                                     & \textbf{UMAP} \\ \hline
\mathbf{$p_{ij}$}    & \begin{tabular}[c]{@{}c@{}}$p_{ij} = (p_{i|j} + p_{j|i})/2n$,\\ $p_{j|i} = \frac{\exp(-\|X_i-X_j\|^2/2\sigma_i^2}{\sum_{k \neq i} \exp(-\|X_i-X_k\|^2/2\sigma_i^2}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$p_{ij} = p_{i|j}+p_{j|i}-p_{i|j} \times p_{j|i}$,\\ $p_{i|j} = exp(-\frac{d(x_i,x_j)-\rho_i}{\sigma_i})$\end{tabular} \\ \hline
\mathbf{$q_{ij}$}    & $q_{ij} = \frac{(1+\|y_i-y_j\|^2)^{-1}}{\sum_{k \neq i} 1+\|y_k-y_i\|^2)^{-1}}$                                       & $q_{ij} = (1+a(y_i-y_j)^{2b})^{-1}$                                                          \\ \hline
\textbf{\text{Loss}} & $\ell = \sum_{i,j, i \neq j} p_{ij}log\big ( \frac{p_{ij}}{q_{ij}} \big )$                                                                                           & $\ell = \sum_i\sum_j \big[-p_{ij} log(q_{ij}) -(1-p_{ij})log(1-q_{ij}) \big] $             \\ \hline
\textbf{\text{Parameters}} & \text{Perplexity} = 2 $\sum_j p_{j|i}\log_2 p_{j|i}$                                                                                         & num of neighbors, $\rho$            \\ \hline
\end{tabular}
\caption{Comparison between t-SNE and UMAP. $p_{ij}$ refers to the high-dimensional distributions on the edges between $x_i$ and $x_j$ given reconstructed knn graphs. $q_ij$ refers to the probability distribution on the low dimension. $x_i$ is the point at the original space X, and $y_i$ is the point at the embedding space Y.}
\label{tab:-umap-n-tsne}
\end{table}


\vspace{5mm}
%==============================
\subsection{Uniform Manifold Approximation \& Projection(UMAP)}
%==============================
UMAP\cite{umap} is known to well preserve the manifold structure in a lower dimensional embedding. There are two key elements that allow UMAP to preserve the manifold structure in a lower dimensional embedding: (1) construct the uniformly distributed simplicial graphs (2) Cross-entropy loss. UMAP first construct the uniformly distributed simplicial graphs and assigns their probability of connection as $p_{i|j} = exp(-\frac{d(x_i,x_j)-\rho_i}{\sigma_i})$, and $p_ij = p_{i|j}+p_{j|i}-p_{i|j} \times p_{j|i}$. Then, we define lower dimensional probability of connectivity as $q_{ij} = (1+a(y_i-y_j)^{2b})^{-1}$. With these probabilities defined, we want to find the lower-dimensional embedding that minimizes the cross entropy between these two distributions. In particular, the loss function can be written as:
$$\ell = \sum_i\sum_j \big[-p_{ij} log(q_{ij}) -(1-p_{ij})log(1-q_{ij}) \big] $$
\begin{enumerate}
        \item For each observation, find the k-nearest neighbors for a given distance metric(typically Euclidean distance).
        \item For each observation, compute $\rho_i$, the minimal distance from the observation $i$ to a neighbor
        \item Compute a scaling parameter $\sigma_i$ for each observation i by solving the equation: $$log_2(k) = \sum_{j=1}^k exp \big( \frac{-max\{0, d(x_i,x_j) - \rho_i\}}{\sigma_i} \big)$$. Intuitively, $\sigma_i$ is used to normalize the distances between every observation and its neighbors to preserve the relative high-dimensional proximities. 
        \item Define the edge weight, $p_{i|j} = exp \big( -\frac{d(x_i,x_j) - \rho_i}{\sigma_i} \big)$
        \item Define a weighted graph, $\mathcal{G}$ whose vertices are the data points($x_i$). The (symmetric) weight of an edge (i,j) applying the product rule is equal to $$p_{ij} = p_{i|j} + p_{j|i} - p_{i|j} \time p_{j|i}$$.
        \item Initialization: initialize $\mathbf{Y}$ using spectral embedding.
        \item Given $\rho_i, \sigma_i$, use binary search to find $a$ and $b$ to define the lower-dimensional probability $q_{ij} = (1+a(y_i-y_j)^{2b})^{-1}$.
\end{enumerate}


\vspace{5mm}
%==============================
\subsection{Dens-NSE, DensMAP}
%==============================
The key modification from t-SNE, UMAP to Dens-NSE, and densMAP\cite{densmap} is that there is an additional regularisation term in the loss function to preserve the local density. We will summarise how this term is defined, and the rest of the loss function and optimization procedure follow the original version.
\begin{enumerate}
    \item \textit{Local radius} represents the expected distance to the nearest neighbors of a given point. The local radius in the original space and embedding space can be defined respectively as $$R_p(x_i) = \frac{1}{\sum_j p_{ij}}\sum_j p_{ij}\|x_i-x_j\|^2, R_q(y_i) = \frac{1}{\sum_j q_{ij}}\sum_j q_{ij}\|y_i-y_j\|^2$$.
    \item We want to preserve this local radius through the dimension reduction procedure. Thus, the objective becomes to find a power-law relationship between $R_P(x_i)$ and $R_Q(y_i)$,i.e. $R_P(x_i) \approx \alpha (R_Q(y_i))^{\beta}$ or equivalently $r_q(y_i) \approx \beta r_p(x_i) + \alpha$, where $r_q(y_i)$ and $r_p(x_i)$ are the logarithms of $R_Q(y_i)$ and $R_P(x_i)$. The goodness-of-fit can be measured by the \textit{correlation coefficient}, which is invariant to the parameter $\alpha$ and $\beta$. $$Corr(r_p, r_q) = \frac{COV(r_p, r_q)}{\sqrt{ \big( Var(r_p)Var(r_q)\big)}}$$ 
    \item The augmented loss becomes $$\ell^{dens} &= \ell - \lambda Corr(r_p, r_q) $$, where $\ell$ refers to the original loss function from UMAP or t-SNE. $\lambda$ determines the relative importance of the density term over the original objective. 
\end{enumerate}


